Knowledge-Centric Templatic Views of Documents

Authors seeking to communicate with broader audiences often share their ideas in various document formats, such as slide decks, newsletters, reports, and posters. Prior work on document generation has generally tackled the creation of each separate format to be a different task, leading to fragmented learning processes, redundancy in models and methods, and disjointed evaluation. We consider each of these documents as templatic views of the same underlying knowledge/content, and we aim to unify the generation and evaluation of these templatic views. We begin by showing that current LLMs are capable of generating various document formats with little to no supervision. Further, a simple augmentation involving a structured intermediate representation can improve performance, especially for smaller models. We then introduce a novel unified evaluation framework that can be adapted to measuring the quality of document generators for heterogeneous downstream applications. This evaluation is adaptable to a range of user defined criteria and application scenarios, obviating the need for task specific evaluation metrics. Finally, we conduct a human evaluation, which shows that people prefer 82% of the documents generated with our method, while correlating more highly with our unified evaluation framework than prior metrics in the literature.

==> tables/gpt4_results.tex <==
\begin{table}[]
\small
\centering
\begin{tabular}{cc|cccc}
 &  & \multicolumn{4}{c}{Simularity Measure} \\
Template & Rep & R-L & M & B & BERTS \\ \hline
\multirow{2}{*}{slides} & $\times$ & 8.3 & \textbf{9.6} & 1.7 & 36.2 \\
 & $\checkmark$ & \textbf{8.4} & 9.1 & \textbf{2.0} & \textbf{38.1} \\
 \hdashline[0.5pt/3pt]
\multirow{2}{*}{blog} & $\times$ & 25.7 & 19.9 & 2.6 & \textbf{82.8} \\
 & $\checkmark$ & \textbf{25.8} & \textbf{20.2} & \textbf{3.1} & 82.7 \\
  \hdashline[0.5pt/3pt]
\multirow{2}{*}{poster} & $\times$ & \textbf{16.4} & \textbf{18.2} & \textbf{4.5} & \textbf{59.8} \\
 & $\checkmark$ & 14.6 & 15.3 & 3.7 & 57.2
\end{tabular}
\caption{\small TAE F1 scores using GPT4 ($\texttt{gpt4-32k}$). We use ROUGE-L (R-L), METEOR (M), BLEU (B) and BERTScore (BERTS) as our similarity measures. For each template, we compare a JSON representation versus skipping the intermediate generation step, maintaining the same style parameters in both settings.
}
\label{tbl:gpt4-results}
\end{table}

==> tables/open-source-results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{ccc|cccc}
 &  &  & \multicolumn{4}{c}{Simularity Measure} \\
task & model & Rep & R-L & M & B & BERTS \\ \hline
\multirow{6}{*}{slides} & \multirow{2}{*}{MS} & times & 0.6 & 0.4 & 0.0 & 28.6 \\
 &  & checkmark & \textbf{4.4} & \textbf{4.6} & \textbf{0.4} & \textbf{30.5} \\ \cline{2-7} 
 & \multirow{2}{*}{MX} & times & 4.8 & 7.3 & 0.5 & 31.8 \\
 &  & checkmark & \textbf{6.7} & \textbf{7.9} & \textbf{1.0} & \textbf{34.0} \\ \cline{2-7} 
 & \multicolumn{1}{l}{\multirow{2}{*}{GPT4}} & \multicolumn{1}{l|}{times} & \multicolumn{1}{l}{8.3} & \multicolumn{1}{l}{\textbf{9.6}} & \multicolumn{1}{l}{1.7} & \multicolumn{1}{l}{36.2} \\
 & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{checkmark} & \multicolumn{1}{l}{\textbf{8.4}} & \multicolumn{1}{l}{9.1} & \multicolumn{1}{l}{\textbf{2.0}} & \multicolumn{1}{l}{\textbf{38.1}} \\ \hline
\multirow{6}{*}{blog} & \multirow{2}{*}{MS} & times & 2.7 & 1.7 & 0.1 & 73.5 \\
 &  & checkmark & \textbf{21.7} & \textbf{16.2} & \textbf{1.7} & \textbf{81.3} \\ \cline{2-7} 
 & \multirow{2}{*}{MX} & times & 22.8 & 15.7 & 2.1 & \textbf{82.6} \\
 &  & checkmark & \textbf{25.6} & \textbf{20.5} & \textbf{3.2} & 82.5 \\ \cline{2-7} 
 & \multicolumn{1}{l}{\multirow{2}{*}{GPT4}} & \multicolumn{1}{l|}{times} & \multicolumn{1}{l}{25.7} & \multicolumn{1}{l}{19.9} & \multicolumn{1}{l}{2.6} & \multicolumn{1}{l}{\textbf{82.8}} \\
 & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{checkmark} & \multicolumn{1}{l}{\textbf{25.8}} & \multicolumn{1}{l}{\textbf{20.2}} & \multicolumn{1}{l}{\textbf{3.1}} & \multicolumn{1}{l}{82.7} \\ \hline
\multirow{6}{*}{poster} & \multirow{2}{*}{MS} & times & 3.2 & 1.8 & 0.2 & 32.2 \\
 &  & checkmark & \textbf{6.0} & \textbf{6.5} & \textbf{1.2} & \textbf{38.1} \\ \cline{2-7} 
 & \multirow{2}{*}{MX} & times & \textbf{10.5} & \textbf{11.4} & \textbf{1.7} & 40.9 \\
 &  & checkmark & 10.4 & 11.0 & 1.5 & \textbf{50.7} \\ \cline{2-7} 
 & \multicolumn{1}{l}{\multirow{2}{*}{GPT4}} & \multicolumn{1}{l|}{times} & \multicolumn{1}{l}{\textbf{16.4}} & \multicolumn{1}{l}{\textbf{18.2}} & \multicolumn{1}{l}{\textbf{4.5}} & \multicolumn{1}{l}{\textbf{59.8}} \\
 & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{checkmark} & \multicolumn{1}{l}{14.6} & \multicolumn{1}{l}{15.3} & \multicolumn{1}{l}{3.7} & \multicolumn{1}{l}{57.2}
\end{tabular}
\end{table}

==> tables/txt_sure.tex <==
\begin{table}
\centering
\small
\begin{tabular}{ll|lll}
Template & \begin{tabular}[c]{@{}l@{}}SURe\\ Format\end{tabular} & R-1 & R-L & \begin{tabular}[c]{@{}l@{}}Bert\\ Score\end{tabular} \\ \hline
\multirow{2}{*}{slides} & JSON & 7.7 & \textbf{7.3} & \textbf{35.1} \\
 & Text & \textbf{7.9} & 7.1 & 34.6 \\ \hdashline[0.5pt/3pt]
\multirow{2}{*}{blog} & JSON & 27.3 & \textbf{25.4} & \textbf{82.7} \\
 & Text & \textbf{28.3} & 24.4 & 82.5 \\ \hdashline[0.5pt/3pt]
\multirow{2}{*}{poster} & JSON & \textbf{14.5} &\textbf{13.5} & \textbf{53.5} \\
 & Text & 11.5 & 10.5 & 46.3
\end{tabular}
\caption{TAE scores comparing the use of the JSON representation of the SURe or passing the text generated in the SURe, using \texttt{gpt35-16k}. We see that in most cases, the JSON representation performs better, indicating the importantance of structure.}
\label{tbl:txt-sure}
\end{table}
